Starling Formation-Flying Optical Experiment: Initial Operations and Flight Results

This paper presents initial flight results for distributed optical angles-only navigation of a swarm of small spacecraft, conducted during the Starling Formation-Flying Optical Experiment (StarFOX). StarFOX is a core payload of the NASA Starling mission, which consists of four CubeSats launched in 2023. Prior angles-only flight demonstrations have only featured one observer and target and have relied upon a-priori target orbit knowledge for initialization, translational maneuvers to resolve target range, and external absolute orbit updates to maintain convergence. StarFOX overcomes these limitations by applying the angles-only Absolute and Relative Trajectory Measurement System (ARTMS), which integrates three novel algorithms. Image Processing detects and tracks multiple targets in images from each satellite's on-board camera. Batch Orbit Determination computes initial swarm orbit estimates from bearing angle batches. Sequential Orbit Determination leverages an unscented Kalman filter to refine swarm state estimates over time. Multi-observer measurements shared over an intersatellite link are seamlessly fused to enable absolute and relative orbit determination. StarFOX flight data presents the first demonstrations of autonomous angles-only navigation for a satellite swarm, including multi-target and multi-observer relative navigation; autonomous initialization of navigation for unknown targets; and simultaneous absolute and relative orbit determination. Relative positioning uncertainties of 1.3% of target range (1$\sigma$) are achieved for a single observer under challenging measurement conditions, reduced to 0.6% (1$\sigma$) with multiple observers. Results demonstrate promising performance with regards to ongoing StarFOX campaigns and the application of angles-only navigation to future distributed missions.

==> Sections/Instructions.tex <==
% Instructions for writing your SmallSat paper

\section*{USING THIS \LaTeX\ TEMPLATE}

This  \LaTeX\ template has been created to assist you in formatting your paper properly.

Fields are enclosed by square brackets, and are used to indicate the proper placement of information. Replace the text in each field, including the square brackets, with the information requested. 

\section*{SUBMISSION PROCEDURES}

Submit your manuscript in PDF format through the Small Satellite Website by the date specified in your acceptance letter.

\section*{MANUSCRIPT SPECIFICATIONS}

\subsection*{Manuscript Length}

The manuscript length is limited to 20 pages, including the abstract, references, and illustrations.  Number all pages sequentially.

\subsection*{Page Specifications}

Use Letter or A4 size paper, using the margins indicated in Table \ref{tab:tab1}. This template is set up for Letter size paper.  

\begin{center}
\fontsize{8}{7.2}\selectfont
\captionof{table}{Page Margins}
\begin{tabular}{|c|c|c|}
    \hline
     \textbf{Margin} & \textbf{Letter} & \textbf{A4} \T\B  \\
     \hline
     Top & 1$^{\prime\prime}$ (2.5 cm) & 1.7$^{\prime\prime}$ (3.43 cm) \T\B\\ 
     \hline
     Bottom & 1$^{\prime\prime}$ (2.5 cm) & 1$^{\prime\prime}$ (2.5 cm) \T\B\\
     \hline
     Left & 1$^{\prime\prime}$ (2.5 cm) & 0.88$^{\prime\prime}$ (2.23 cm) \T\B\\
     \hline
     Right & 1$^{\prime\prime}$ (2.5 cm) & 0.88$^{\prime\prime}$ (2.23 cm) \T\B\\
     \hline
\end{tabular}
\label{tab:tab1}
\end{center}

\subsection*{Paper Identification}

Use the field in the upper right corner of the first page to enter your paper number (see your acceptance letter), in bold 14-point Computer Modern (or similar) typeface, flush with the right margin.

\subsection*{Title}

Use the field on the second line of the first page to type your paper title across both columns, in bold 12-point Computer Modern (or similar) typeface. Spell out all acronyms that are not commonly known. Capitalize the first letter of all words in the title, except articles and prepositions.

\subsection*{Authors and Affiliations}

Center authors' names across both columns, one line below the title, as shown above. Please use full names of all authors rather than initials.  Omit titles or degrees such as Dr., Prof., Ph.D, etc. On separate lines, type the author's affiliation, address and phone number, and email address. Double-space between each author's information. Authors with the same affiliation should be listed together, as shown. 

\subsection*{Page Footer}

The footer should fall within the bottom margin, with a thin line separating the footer from the body of the paper, as shown in this template.  The footer should contain the last name of the first author (left aligned), the page number (centered), and the name of the conference (right aligned).  Please enter the last name of the first author and the two-digit conference number in the appropriate fields.

\section*{CONTENT LAYOUT}

\subsection*{Body Text}

Use 10-point Computer Modern (or similar) typeface for the body text, arranged in two-column format. Paragraphs should be indented, single-spaced, and fully justified.

\subsection*{Headings}

Primary headings should be bold 10-point Computer Modern (or similar) typeface, using all capitals.

Subheadings should be bold italic 10-point Computer Modern (or similar) typeface. Capitalize the first letter of all words, excluding articles and prepositions.

\subsection*{Illustrations}

Figures and tables will be reproduced exactly as submitted, and should be numbered sequentially. Incorporate all figures and tables in place, ideally immediately following the paragraph in which they are first referenced. Illustrations may fit into one column (Figure \ref{fig:cryo}, Tables \ref{tab:tab1} and \ref{tab:tab2}) or may extend across both columns (Figure \ref{fig:states}). Company logos and identification numbers are not permitted in illustrations.

\begin{Figure}
    \centering
    \includegraphics[width = 5cm]{Images/fig1.png}
    \captionof{figure}{Cryocooler Assembly}
    \label{fig:cryo}
\end{Figure}

Below each figure, use the \texttt{\textbackslash captionof} environment to center a caption in bold 10-point Computer Modern (or similar) typeface, capitalizing the first letter of all words except articles and prepositions.  All text within figures, including axis labels and legends, should be 8 pt or larger.  Line widths for axes and data should be at least 0.5 pt. Each figure should be prepared for 100\% reproduction to avoid problems arising from large reductions in size. The \texttt{\textbackslash Figure} environment with \texttt{\textbackslash centering} works well for single-column figures (Figure \ref{fig:cryo}), and the \texttt{\textbackslash figure*} environment with \texttt{\textbackslash centering} for two-column figures (Figure \ref{fig:states}).  

\begin{center}
\fontsize{8}{7.2}\selectfont
{\tabulinesep=1.1mm
\captionof{table}{Style Specifications}
\label{tab:tab2}
\begin{tabu}{|p{1.5cm}|p{0.8cm}|p{1.0cm}|p{2.8cm}|}
    \hline
     \textbf{Style} & \textbf{Font Size} & \textbf{Weight} & \textbf{Capitalization}\\
     \hline
     Paper Number & 14 pt & Bold & To match assigned number\\
     \hline 
     Title & 12 pt & Bold & First letter of all words, except articles and prepositions\\
     \hline 
     Authors & 10 pt & Normal & Normal\\ 
     \hline
     Primary Headings & 10 pt & Bold & All capitals\\
     \hline
     Subheadings & 10 pt & Bold Italic & First letter of all words, except articles and prepositions\\
     \hline
     Body Text & 10 pt & Normal & Normal\\
     \hline
     Illustration Captions & 10 pt & Bold & First letter of all words, except articles and prepositions \\
     \hline
     Illustration Text & 8 pt & Normal & Normal\\
     \hline
\end{tabu}}
\end{center}

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth, trim=65 55 65 110, clip]{Images/fig2.pdf}
    \captionof{figure}{States plot}
    \label{fig:states}
\end{figure*}

Above each table, use the \texttt{\textbackslash captionof} environment to center a caption in bold 10-point Computer Modern (or similar) typeface, capitalizing the first letter of all words except articles and prepositions. All text within tables should be 8 pt or larger.  The \texttt{\textbackslash tabular} (Table \ref{tab:tab1}) and \texttt{\textbackslash tabu} (Table \ref{tab:tab2}) environments work well for tables when coupled with the \texttt{\textbackslash center} environment. 

\subsection*{Equations}

Left flush equations and number them sequentially. Enclose equation numbers in parentheses flush to the right margin.

Use standard symbols and abbreviations in equations, and define all variables. For example, the Reynolds number for flow through a tube of diameter $D$ is given by
\begin{equation}
    \textrm{Re} = \frac{uD}{\nu}
\end{equation}
where $u$ is the flow speed and $\nu$ is the kinematic viscosity of the fluid.  

Lengthy equations may extend across both columns. 

\subsection*{Acknowledgments}

Acknowledgments for technical, financial, or other forms of support should just precede the references.

\subsection*{Footnotes}

Including information in the text is preferred over creating footnotes. In tables, the following reference marks should be used if footnotes are needed: *, **, $\dagger$, etc. 

\subsection*{References} 

List all bibliographical references at the end of the paper, numbered sequentially in the order cited, and formatted as shown in the bibliography below.  Use superscript citations as shown at the end of this sentence.\cite{bombelli_economic_2003, Goldstein_Greening, anderson}


